Time Weaver: A Conditional Time Series Generation Model

Imagine generating a city's electricity demand pattern based on weather, the presence of an electric vehicle, and location, which could be used for capacity planning during a winter freeze. Such real-world time series are often enriched with paired heterogeneous contextual metadata (e.g., weather and location). Current approaches to time series generation often ignore this paired metadata. Additionally, the heterogeneity in metadata poses several practical challenges in adapting existing conditional generation approaches from the image, audio, and video domains to the time series domain. To address this gap, we introduce TIME WEAVER, a novel diffusion-based model that leverages the heterogeneous metadata in the form of categorical, continuous, and even time-variant variables to significantly improve time series generation. Additionally, we show that naive extensions of standard evaluation metrics from the image to the time series domain are insufficient. These metrics do not penalize conditional generation approaches for their poor specificity in reproducing the metadata-specific features in the generated time series. Thus, we innovate a novel evaluation metric that accurately captures the specificity of conditional generation and the realism of the generated time series. We show that TIME WEAVER outperforms state-of-the-art benchmarks, such as Generative Adversarial Networks (GANs), by up to 30% in downstream classification tasks on real-world energy, medical, air quality, and traffic datasets.

==> figures_latex/distro.tex <==
\begin{figure*}[!ht]
\centering
  \includegraphics[width=1\textwidth]{figures/two_row_distribution.pdf}
\vspace{-2em}
\caption{\small{\textbf{The data distribution learned by \timeweaver \space accurately captures the timestep magnitudes and the frequency profile of the dataset.} In this figure, we transform both real and synthesized time series datasets into frequency distributions over their respective values. These histogram plots illustrate the distribution of samples generated by the \timeweaver \space models closely aligns with the distribution of real samples, whereas the GAN model lags behind in accurately capturing the real dataset. }}
\vspace{-1em}
\label{fig:qual_distribution}
\end{figure*}

==> figures_latex/ecg_tsne_qualitative.tex <==
\begin{figure*}[h!]
\centering
 \includegraphics[width=1.0\textwidth]{figures/qualitative/ecg_tsne_classifier_guidance_20.0.pdf}
     
\caption{\small{\textbf{t-SNE plot showing the original and the synthesized dataset.} Our approach effectively captures the original data distribution. We elucidate this using t-SNE plots generated with the samples from the original dataset and the generated samples for the same set of conditions, for all the $12$ channels in the ECG dataset. }}
\label{fig:ecg_qualitative}
\end{figure*}

==> figures_latex/electricity_qualitative.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=1.0\textwidth]{figures/qualitative/waveforms_qualitative.pdf}
\caption{\small{\textbf{\timeweaver \space provides near perfect samples for synthetic datasets.} }}
\label{fig:qualitative}
\end{figure*}


==> figures_latex/ftsd_results.tex <==
\begin{figure}
\centering
 \includegraphics[width=0.75\columnwidth]{figures/fid_scores/label_flipping.pdf}
  % \includegraphics[width=1.2\textwidth]{figures/qualitative/distro.pdf}
  % \includegraphics[width=1.2\textwidth]{figures/qualitative/fft-distro.pdf}
  
     
\caption{\small{\textbf{Our proposed metric is robust to label flipping attacks.}}}
\label{fig:ftsd_qualitative}
\end{figure}

==> figures_latex/toy_example.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/toy_example.png}
    \caption{\small{\textbf{Synhesizing Time series from metadata using \timeweaver} With just the metadata condition $\condition$, (left), \timeweaver \space can generate a realistic time series sample $\timeseries$ (right). In the example above, \timeweaver \space generates the electricity demand just from the following conditions - \textit{User: ABC} and the month \textit{May}. The plot on the right shows how close the synthesized time series (orange) is to the real time series (green), thus showing \timeweaver's ability to synthesize time series patterns specific to the metadata. } }
\end{figure}

==> figures_latex/tsne.tex <==
% \begin{figure*}[h!]
% \centering
%  \includegraphics[width=1.2\textwidth]{figures/qualitative/tsne-combined-for-all.pdf}
%   % \includegraphics[width=1.2\textwidth]{figures/qualitative/distro.pdf}
%   % \includegraphics[width=1.2\textwidth]{figures/qualitative/fft-distro.pdf}
  
     
% \caption{\small{\textbf{t-SNE plot showing the distribution of the real and the synthetic datasets across different domains.} Our approach effectively captures the original data distribution. We elucidate this using t-SNE plots generated with the samples from the original dataset and the synthesized samples for the same set of metadata.}}
% \label{fig:tsne_qualitative}
% \end{figure*}

==> figures_latex/visual_results.tex <==
\begin{figure*}[thpb]
% \vskip 0.2in
\centering

\begin{subfigure}[b]{0.4\columnwidth}
     % \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/cc_cd_pmax.eps}
    \caption{\footnotesize{Safe states - constant delay}}
    \label{fig:simulation_results_a}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.4\columnwidth}
     % \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/cc_rd_pmax.eps}
    \caption{\footnotesize{Safe states - random delay}}
    \label{fig:simulation_results_b}
 \end{subfigure}
  \hfill
 \begin{subfigure}[b]{0.9\columnwidth}
     \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/cc_emp.eps}
    \caption{\footnotesize{Quantitative results}}
    \label{fig:simulation_results_c}
 \end{subfigure}
 \begin{subfigure}[b]{0.4\columnwidth}
     \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/gw_cd_pmax.eps}
    \caption{\footnotesize{Safe states - constant delay}}
    \label{fig:simulation_results_d}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.4\columnwidth}
     \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/gw_rd_pmax.eps}
    \caption{\footnotesize{Safe states - random delay}}
    \label{fig:simulation_results_e}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.9\columnwidth}
     \centering
     \includegraphics[width=1.0\textwidth]{figures/simulation/gw_emp_RAL.eps}
    \caption{\footnotesize{Quantitative results}}
    \label{fig:simulation_results_f}
 \end{subfigure}
     
\caption{\textbf{Shielding leads to safe networked control in simulations.} .}
% Figs. \ref{fig:simulation_results_c} and \ref{fig:simulation_results_f} show that as latency increases, the system tends to be conservative, leading to increased distances in the car-following scenario, and increased number of ties in the grid world case.}}
%. Figs. \ref{fig:simulation_results_e} and \ref{fig:simulation_results_f} show that as the delay increases, the networked control system is conservative.} \sai{The random delay case incorporates the latency transition model in the networked MDP, so an initial state should be safe only with respect to the expected WiFi latency and not the maximum latency, which is the constant delay case. Hence, we observe that aggressive initialization is possible for the random delay case and not for the constant delay case. Figs. \ref{fig:simulation_results_c} and \ref{fig:simulation_results_f} show the task performance of our safe networked control approach in both the environments. In general, with increasing latency, the system tends to be conservative, increased minimum distance in the car-following scenario, and increased number of ties in the grid world case.}}}
\label{fig:simulation_results}
\vspace{-1em}
\end{figure*}

==> sections/broader_impact.tex <==
This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.



==> sections/checklist.tex <==
% For the paper checklist
\newcommand{\answerYes}[1]{{\color{blue}{[Yes]#1}}}
\newcommand{\answerNo}[1]{{\color{red}{[No]#1}}}
\newcommand{\answerNA}[1]{{\color{red}{[N/A]#1}}}
\newcommand{\answerTODO}[1]{{\color{red}{\bf[TODO]}}}

\noindent \textbf{Paper Submission Checklist}

\noindent \textbf{Student Name: Sai, Somi, Oguzhan} \newline
\noindent \textbf{Peer Reviewer Name:}  \newline
\noindent \textbf{Paper Title: \textsc{TimeWeaver}: A Conditional Timeseries Synthesis Model} \newline
\noindent \textbf{Date: 12/15/2023} \newline

\begin{enumerate}
    \item Did you spell check and grammar check the full document, using Grammarly if needed?
    \answerYes{}
    \item Did you organize the LaTeX files according to the sample paper guide, including naming the file appropriately, organizing sections etc.? \answerYes{}
  \item Did you make sure all plots are legible, in at least 20 point font, and ideally use the lab plotting tools/guidelines? \answerYes{}
  \item Did you have another student in the lab peer review your paper for clarity, typos, wrong notation etc.? Send an email to Sandeep (CC'ing both students) with the paper draft. \answerNo{}
  \item Did you make sure all references have the book/conference venue, not just the author and title? \answerNo{}
  \item Did you use the common reference files in the lab GIT, making sure to put our internal papers in ref/SwarmLabPubs.bib and all other papers in ref/external.bib? \answerYes{}
  \item Did you outline your paper and place the DARPA Heilmeier Catechism question answers at the top of the outline? \answerNo{}
\end{enumerate}


\newpage


==> tables_latex/electricity_quantitative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{sc}
\begin{tabular}{lllll}
\hline
Approach                                                                     & \begin{tabular}[c]{@{}l@{}}Mean \\ $l_1$ error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Median \\ $l_1$ error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mean \\ \% error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Median \\ \% error\end{tabular} \\ \hline
% CVAE                                                                         &                                                          &                                                            &                                                          &                                                            \\ \hline
% CTGAN                                                                        &                                                          &                                                            &                                                          &                                                            \\ \hline
% DoppleGANger                                                                 &                                                          &                                                            &                                                          &                                                            \\ \hline
DDPM                                                                         & 0.0412                                                   & 0.0078                                                     & 142.11                                                   & 4.8                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}DDPM with learned \\ condition input\end{tabular} & \textbf{0.0409}                                                   & \textbf{0.00565}                                                    & \textbf{64.89}                                                    & \textbf{3.52}                                                       \\ \hline
\end{tabular}%
\end{sc}
}
\caption{\small{\textbf{Quantitative results for the electricity dataset.} Our approach outperforms other GAN and VAE-based conditional generation baselines on $l_1$ and \% error for the electricity dataset.}}
\label{tab:electricity_quantitative}
\end{table}

==> tables_latex/imputation_electricity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{sc}
\begin{tabular}{lllll}
\hline
Approach     & \begin{tabular}[c]{@{}l@{}}MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}RMSE\end{tabular} & \begin{tabular}[c]{@{}l@{}}MRE\end{tabular} \\ \hline

OURS         & \textbf{0.121}                                                   & \textbf{0.242}                                                    & 0.224                                                        \\ \hline
SSSD         & 0.532           & 0.821           & 0.285 \\ \hline

CSDI         & 0.278           & 2.37            & \textbf{0.149}

\end{tabular}%
\end{sc}
}
\caption{\small{\textbf{Quantitative results for the waveforms dataset.} Our approach outperforms other GAN and VAE-based conditional generation baselines on $l_1$ and \% error for the waveforms dataset.  }}
\label{tab:waveforms_quantitative}
\end{table}

==> tables_latex/quant_comp_final.tex <==

\begin{table*}
\centering
% \resizebox{0.8\textwidth}{!}{%
\scalebox{0.80}{
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccc}
\hline
{Approach} & \multicolumn{2}{c}{Air Quality} & \multicolumn{2}{c}{ECG} & \multicolumn{2}{c}{Traffic} & \multicolumn{2}{c}{Electricity} \\ 
                          & J-FTSD \(\downarrow\) & TSTR \(\uparrow\)      & J-FTSD \(\downarrow\)    & TSTR \(\uparrow\)  & J-FTSD \(\downarrow\)     & TSTR \(\uparrow\)    & J-FTSD \(\downarrow\)         & TSTR \(\uparrow\)       \\ \hline
WaveGAN \\
\cite{donahue2019wavegan}  & 13.38$\pm$0.01 & 0.63$\pm$0.01 & 9.55$\pm$0.01 & 0.65$\pm$0.001 & 25.69$\pm$0.01 & 0.54$\pm$0.01 & 7.82$\pm$0.002 & 0.57$\pm$0.007 \\ \hline
Pulse2Pulse \\
\cite{thambawita2021pulse2pulse}  & 23.48$\pm$0.02 & 0.61$\pm$0.02 & 13.49$\pm$0.04 & 0.63$\pm$0.03 & 17.70$\pm$0.002 & 0.52$\pm$0.03 & 2.8$\pm$0.01 & 0.71$\pm$0.004 \\ \hline
% UNet-1D    & 7.32$\pm$0.04 & 0.66$\pm$0.01 & 12.9$\pm$0.1 & 0.71$\pm$0.01 & 0.36$\pm$0.03 & 0.65$\pm$0.02 & 1.19$\pm$0.008 & 0.77$\pm$0.001  \\ \hline
\timeweaver-CSDI   & \textbf{2.15$\pm$0.04} & \textbf{0.75$\pm$0.03} & 7.25$\pm$0.09 & 0.83$\pm$0.001 & 0.53$\pm$0.01 & \textbf{0.66$\pm$0.06} & \textbf{0.6$\pm$0.003} & \textbf{0.78$\pm$0.001}  \\ \hline
\timeweaver-SSSD    & 8.17$\pm$0.17 & 0.64$\pm$0.04 & \textbf{5.43$\pm$0.1} & \textbf{0.85$\pm$0.007} & \textbf{0.36$\pm$0.03} & 0.65$\pm$0.07 & 1.19$\pm$0.008 & 0.77$\pm$0.001  \\ \hline


\end{tabular}
\end{sc}
\end{small}
}
\vspace{-0.5em}
\caption{\textbf{\timeweaver \space outperforms \ac{gan}-based approaches on \ac{jftsd} and \ac{tstr} metrics}. The table shows the performance of all the models (rows) on specified datasets (columns). The \timeweaver \space variants significantly outperform \acp{gan} on the \ac{jftsd} and TSTR metrics. Our experimental findings also confirm that lower \ac{jftsd} scores correspond to higher \ac{auc} (TSTR) scores when tested on the original test dataset, showcasing the utility of our proposed \ac{jftsd} metric in evaluating the quality of the generated data distribution. \textcolor{blue}{We report both metrics' mean and standard deviation averaged over six seeds.}}
\vspace{-1em}
\label{tab:quant_comp}
\end{table*}

==> tables_latex/tstr.tex <==
\begin{table*}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{sc}
\begin{tabular}{lllllllll}
\hline
Approach        & \begin{tabular}[c]{@{}l@{}}Air Quality \end{tabular} & \begin{tabular}[c]{@{}l@{}}ECG\end{tabular} & \begin{tabular}[c]{@{}l@{}}Traffic\end{tabular} & \begin{tabular}[c]{@{}l@{}}Electricity\end{tabular} \\ \hline
Pulse2Pulse \cite{thambawita2021pulse2pulse}  & TBD   & TBD  & TBD  & TBD \\ \hline
\timeweaver-CSDI   & \textbf{0.77}   & TBD  & TBD  & \textbf{0.8422} \\ \hline
\timeweaver-SSSD    & 0.64   & TBD  & TBD  & 0.83 \\ \hline

\end{tabular}%
\end{sc}
}
\caption{\small{\textbf{The trend for FTSD matches with the trend for Train on Synthetic and Test on Real.} We report the performance of classification models that were trained on synthetic data generated by the baseline approaches and \timeweaver, \space and tested on the original test dataset. For classification, we choose one of the categorical conditions from the metadata that is not time varying. For example, we have chosen ``month'' for the electricity dataset, ``city'' for the air-quality dataset, and ``diagnosed disease'' for the ECG dataset. Our experimental findings indicate that lower FTSD scores correspond to higher Area Under the Curve (AUC) scores when tested on the original test dataset.}}
\label{tab:ecg_auc_table}
\end{table*}

==> tables_latex/waveforms_quantitative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{sc}
\begin{tabular}{lllll}
\hline
Approach     & \begin{tabular}[c]{@{}l@{}}Mean \\ $l_1$ error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Median \\ $l_1$ error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mean \\ \% error\end{tabular} & \begin{tabular}[c]{@{}l@{}}Median \\ \% error\end{tabular} \\ \hline
% CVAE         &                                                          &                                                            &                                                          &                                                            \\ \hline
% CTGAN        &                                                          &                                                            &                                                          &                                                            \\ \hline
% DoppleGANger &                                                          &                                                            &                                                          &                                                            \\ \hline
DDPM         & 0.0144                                                   & 0.0046                                                     & 17.86                                                    & 1.85                                                       \\ \hline
\end{tabular}%
\end{sc}
}
\caption{\small{\textbf{Quantitative results for the waveforms dataset.} Our approach outperforms other GAN and VAE-based conditional generation baselines on $l_1$ and \% error for the waveforms dataset.  }}
\label{tab:waveforms_quantitative}
\end{table}
